Compressed Decentralized Proximal Stochastic Gradient Method for Nonconvex Composite Problems with Heterogeneous Data

We first propose a decentralized proximal stochastic gradient tracking method (DProxSGT) for nonconvex stochastic composite problems, with data heterogeneously distributed on multiple workers in a decentralized connected network. To save communication cost, we then extend DProxSGT to a compressed method by compressing the communicated information. Both methods need only $\mathcal{O}(1)$ samples per worker for each proximal update, which is important to achieve good generalization performance on training deep neural networks. With a smoothness condition on the expected loss function (but not on each sample function), the proposed methods can achieve an optimal sample complexity result to produce a near-stationary point. Numerical experiments on training neural networks demonstrate the significantly better generalization performance of our methods over large-batch training methods and momentum variance-reduction methods and also, the ability of handling heterogeneous data by the gradient tracking scheme.

==> Decentralized_nonconvex_nonsmooth_ arXiv/algorithms.tex <==

\section{Decentralized Algorithms}\label{sec:alg}

In this section, we give our decentralized algorithms for solving \eqref{eq:decentralized_problem} or equivalently \eqref{eq:problem_original}. To perform neighbor communications, we introduce a mixing (or gossip) matrix $\W$ that satisfies the following standard assumption.
\begin{assumption}[Mixing matrix] \label{assu:mix_matrix} We choose a mixing matrix $\W$ such that
% \JC{It appears that $\W$ is assumed to be symmetric? We do not need}
\vspace{-1.5mm}
\begin{enumerate}
\item [(i)] $\W$ is doubly stochastic: $\W\1 = \1$ and $\1^\top \W = \1^\top$;
\item [(ii)] $\W_{ij} = 0$ if $i$ and $j$ are not neighbors to each other;
\item [(iii)] $\mathrm{Null}(\W-\I) = \mathrm{span}\{\1\}$ and $\rho \triangleq \|\W - \J\|_2 < 1$.
\end{enumerate}
\vspace{-2mm}
\end{assumption}
The condition in (ii) above is enforced so that \emph{direct} communications can be made only if two nodes (or workers) are immediate (or 1-hop) neighbors of each other. The condition in (iii) can hold if the graph $\hG$ is connected. The assumption $\rho < 1$ is critical to ensure contraction of consensus error. 

% \YX{Mention a few examples of $\W$ by referring to existing papers.}
The value of $\rho$ depends on the graph topology.   
\cite{koloskova2019decentralized} gives three commonly used examples: when uniform weights are used between nodes, $\W = \J$ and $\rho = 0$ for a fully-connected graph (in which case, our algorithms will reduce to centralized methods), $1-\rho = \Theta(\frac{1}{n})$ for a 2d torus grid graph where every node has 4 neighbors, and $1-\rho = \Theta(\frac{1}{n^2})$ for a ring-structured graph. %each node has two neighbors and $\rho^{-1} = \hO(n^2)$, for a 2d-torus each node has 4 neighbors and $\rho^{-1} = \hO(n)$, for a fully connected graph each node connects with all others and $\rho^{-1} = \hO(1)$. 
More examples can be found in \cite{nedic2018network}.

% The mixing matrix $\W\in  \bbR^{n\times n}$ and the identity matrix as $\I\in  \bbR^{n\times n}$. We will denote the value of $\W$ at $(j,i)$ position as $\W_{ji}$. 


% {\color{blue}i suggest to add some captions to present these details.}

\subsection{Non-compreseed Method}

With the mixing matrix $\W$, we propose a decentralized proximal stochastic gradient method with gradient tracking (DProxSGT) for \eqref{eq:decentralized_problem}. The pseudocode is shown in Algorithm~\ref{alg:DProxSGT}. 
In every iteration $t$, each node $i$ first computes a local stochastic gradient $\nabla F_i(\vx_i^{t},\xi_i^{t})$ by taking a sample $\xi_i^{t}$ from its local data distribution $\mathcal{D}_i$, then performs gradient tracking in \eqref{eq:y_half_update} and neighbor communications of the tracked gradient in \eqref{eq:y_update}, and finally takes a proximal gradient step in \eqref{eq:x_half_update} and mixes the model parameter with its neighbors in \eqref{eq:x_1_update}.

\begin{algorithm}[tb]
   \caption{DProxSGT}\label{alg:DProxSGT}
\begin{algorithmic}
   \small{ \STATE Initialize $\vx_i^{0}$ and set $\vy_i^{-1}=\0$, $\nabla F_i(\vx_i^{-1},\xi_i^{-1}) =\0$,   $\forall i\in\hN$. %=1, 2, \ldots, n$.  
   \FOR{$t=0, 1, 2, \ldots, T-1$} 
   \STATE \hspace{-0.1cm}\textbf{all} nodes $i=1, 2, \ldots, n$ do the updates \textbf{in parallel:}
   \STATE obtain one random sample $\xi_i^t$, compute a stochastic gradient $\nabla F_i(\vx_i^{t},\xi_i^{t})$, and perform 
   \vspace{-0.2cm}
       \begin{gather}
            	\vy_i^{t-\frac{1}{2}} =  \vy_i^{t-1}  +  \nabla F_i(\vx_i^{t},\xi_i^{t}) - \nabla F_i(\vx_i^{t-1},\xi_i^{t-1}),\label{eq:y_half_update}
            	\\
            	\vy_i^t =  \textstyle \sum_{j=1}^n \W_{ji} \vy_j^{t-\frac{1}{2}},\label{eq:y_update}\\
            	\vx_i^{t+\frac{1}{2}} =\prox_{\eta r} \left(\vx_i^t - \eta \vy_i^{t}\right),\label{eq:x_half_update}
            	\\
            	\vx_i^{t+1} =  \textstyle \sum_{j=1}^n \W_{ji}\vx_j^{t+\frac{1}{2}}. \label{eq:x_1_update}
          \vspace{-0.2cm}   
    	\end{gather}   
   \ENDFOR}
\end{algorithmic}
\end{algorithm}
\vspace{-0.1mm}
 

Note that for simplicity, we take only one random sample $\xi_i^{t}$ in Algorithm \ref{alg:DProxSGT} but in general, a mini-batch of random samples can be taken, and all theoretical results that we will establish in the next section still hold. We emphasize that we need only $\mathcal{O}(1)$ samples for each update. This is different from ProxGT-SA in \cite{xin2021stochastic}, which shares a similar update formula as our algorithm but needs a very big batch of samples, as many as $\mathcal{O}(\frac{1}{\epsilon^2})$, where $\epsilon$ is a target tolerance. A small-batch training can usually generalize better than a big-batch one \cite{lecun2012efficient, keskar2016large} on training large-scale deep learning models. Throughout the paper, we make the following standard assumption on the stochastic gradients.

%Here, $\xi_i^{t}$ denotes the random samples taken from the data on node $i$ at iteration $t$, and it
%can be a mini-batch of samples. We assume $\xi_i^t$ and the stochastic gradients $\nabla F_i(\vx_i,\xi_i)$ satisfy the following assumption.
\begin{assumption}[Stochastic gradients] \label{assu:stoc_grad}
We assume that 
\vspace{-1.5mm}
\begin{itemize}
    \item[(i)] The random samples $\{\xi_i^t\}_{i\in \hN, t\ge 0}$ are independent. %for all $i\in \hN, t\geq 0$.
    \item[(ii)] %The stochastic gradients are unbiased and have bounded variance, i.e., 
    There exists a finite number $\sigma\ge0$ such that for any $i\in \hN$ and $\vx_i\in\dom(r)$, %$\xi_i\sim \mathcal{D}_i$ and $i\in[n]$,  
    \begin{gather*}  
    \bbE_{\xi_i}[\nabla F_i(\vx_i,\xi_i)]  = \nabla f_i(\vx_i),\\ 
    \bbE_{\xi_i}[\|\nabla F_i(\vx_i,\xi_i)-\nabla f_i(\vx_i)\|^2] \leq \sigma^2.
     \end{gather*}  
\end{itemize}
\vspace{-2mm}
\end{assumption}
  

% \YX{Let us write the algorithm from the point view of each worker. The current updates are some equivalent writing and let's use those in the analysis. Or explain how to implement the current updates in a decentralized way. The former is better. We should also state in the algorithm to take samples on each worker. Then explain that we can take a mini-batch of samples.}

% \YX{Mention that \eqref{eq:y_half_update} is the gradient tracking step (give the reference). Emphasize that it is critical to handle heterogeneous data. With the gradient tracking, we do not need to assume strong assumptions like bounded gradient, or data similarity (give some references).}

The gradient tracking step in \eqref{eq:y_half_update} %-\eqref{eq:y_update} are 
is critical to handle heterogeneous data 
% \JC{Can we elaborate how?}
\cite{di2016next,nedic2017achieving,lu2019gnsd,pu2020distributed,sun2020improving,xin2021stochastic,song2021optimal,mancino2022proximal,zhao2022beer,DBLP:journals/corr/abs-2202-00255,song2022compressed}.
In a deterministic scenario where $\nabla f_i(\cdot)$ is used instead of $\nabla F_i(\cdot, \xi)$, for each $i$, the tracked gradient $\vy_i^t$ can converge to the gradient of the global function $\frac{1}{n}\sum_{i=1}^n f_i(\cdot)$ at $\bar\vx^t$, and thus all local updates move towards a direction to minimize the \emph{global} objective. When stochastic gradients are used, the gradient tracking can play a similar role and make $\vy_i^t$ approach to the stochastic gradient of the global function. 
%The tracked gradient $\vy_i$ estimates the average gradients over all nodes, thus directs $\vx_i$ toward the optimal model parameters of $\phi(\vx)$ in \eqref{eq:x_half_update}. If directly use $\nabla F_i(\vx_i^{t},\xi_i^{t})$ in \eqref{eq:x_half_update}, 
%even $\vx_i^t$ are identical at iteration $t$, $\vx_i^t$ may still move towards dramatically different directions indicated by local stochastic gradients, resulting in different $\vx_i^{t+1}$ for the next iteration $t+1$.
%Also theoretically, 
With this nice property of gradient tracking, we can guarantee convergence without strong assumptions that are made in existing works, such as bounded gradients  \cite{koloskova2019decentralized,koloskova2019decentralized-b, taheri2020quantized, singh2021squarm}  and bounded data similarity over nodes \cite{lian2017can, tang2018communication, tang2019deepsqueeze, vogels2020practical, wang2021error}.
 


\subsection{Compressed Method}
% \YX{Explain what we need to communicate in Algorithm 1. Then say communications are becoming bottleneck for distributed training by GPUs, so in order to save communication cost, we further propose a compressed algorithm.}
In DProxSGT, each worker needs to communicate both the model parameter and tracked stochastic gradient with its neighbors at every iteration. Communications have become a bottleneck for distributed training on GPUs. In order to save the communication cost, we further propose a compressed version of DProxSGT, named CDProxSGT. The pseudocode is shown in Algorithm \ref{alg:CDProxSGT}, where $Q_\vx$ and $Q_\vy$ are two compression operators.

\begin{algorithm}[tb]
\caption{CDProxSGT}\label{alg:CDProxSGT}
\begin{algorithmic}
  \small{\STATE Initialize  $\vx_i^{0}$; set 
  $\vy_i^{-1}=\underline\vy_i^{-1}=\nabla F_i(\vx_i^{-1}, \xi_i^{-1})=\underline\vx_i^{0} =\0$, $\forall i\in\hN$. %=1, 2, \ldots, n$.
  \FOR{$t=0, 1, 2, \ldots, T-1$}
     \STATE \hspace{-0.1cm}\textbf{all} nodes $i=1, 2, \ldots, n$ do the updates \textbf{in parallel:}
     \vspace{-0.2cm}
         \begin{gather}
    	\vy_i^{t-\frac{1}{2}} =  \vy_i^{t-1} + \nabla F_i(\vx_i^{t},\xi_i^{t}) - \nabla F_i(\vx_i^{t-1},\xi_i^{t-1}),\label{eq:alg3_1}\\
        \underline\vy_i^{t} = \underline\vy_i^{t-1} + Q_\vy\big[\vy_i^{t-\frac{1}{2}} - \underline\vy_i^{t-1}\big], \label{eq:alg3_2}\\
        \vy_i^{t} = \vy_i^{t-\frac{1}{2}} +\gamma_y  \left(\textstyle \sum_{j=1}^n \W_{ji} \underline\vy_j^{t}-\underline\vy_i^{t}\right), \label{eq:alg3_3}\\
    	\vx_i^{t+\frac{1}{2}} =\prox_{\eta r} \left(\vx_i^t - \eta \vy_i^{t}\right), \label{eq:alg3_4}\\
    	\underline\vx_i^{t+1} = \underline\vx_i^{t} + Q_\vx\big[\vx_i^{t+\frac{1}{2}} - \underline\vx_i^{t}\big], \label{eq:alg3_5}\\
    	\vx_i^{t+1} = \vx_i^{t+\frac{1}{2}}+\gamma_x\Big(\textstyle  \overset{n}{\underset{j=1}\sum} \W_{ji} \underline\vx_j^{t+1}-\underline\vx_i^{t+1}\Big).\label{eq:alg3_6}
     \vspace{-0.2cm}
     \end{gather}    
   \ENDFOR}
\end{algorithmic}
\end{algorithm}
\vspace{-0.1mm}

 

% \YX{The given update does not look to have low communication cost. Explain the equivalent implementation form that only communicates the compressed vectors.}
In Algorithm \ref{alg:CDProxSGT}, each node communicates the non-compressed vectors $\underline\vy_i^{t}$ and $\underline\vx_i^{t+1}$  with its neighbors in \eqref{eq:alg3_3} and \eqref{eq:alg3_6}. We write it in this way for ease of read and analysis. For efficient and \emph{equivalent} implementation, %the nodes 
we do not communicate 
$\underline\vy_i^{t}$ and $\underline\vx_i^{t+1}$ directly but the compressed residues  $Q_\vy\big[\vy_i^{t-\frac{1}{2}} - \underline\vy_i^{t-1}\big]$ and $Q_\vx\big[\vx_i^{t+\frac{1}{2}} - \underline\vx_i^{t}\big]$, explained as follows. 
Besides $\vy_i^{t-1}$, $\vx_i^{t}$, $\underline\vy_i^{t-1}$ and $\underline\vx_i^{t}$, each node also stores $\vz_i^{t-1}$ and $\vs_i^{t}  $ which record $\sum_{j=1}^n \W_{ji} \underline\vy_i^{t-1}$ and $\sum_{j=1}^n \W_{ji} \underline\vx_i^{t}$. For the gradient communication, each node $i$ initializes $\vz_i^{-1} = \0$, and then at each iteration $t$, 
after receiving $Q_\vy\big[\vy_j^{t-\frac{1}{2}} - \underline\vy_j^{t-1}\big]$ from its neighbors, it updates $\underline\vy_i^{t}$ by \eqref{eq:alg3_2}, and $\vz_i^{t}$ and $\vy_i^t$ by 
\vspace{-0.2cm} 
\begin{align*}
  \vz_i^{t} =&~ \textstyle \vz_i^{t-1} + \sum_{j=1}^n \W_{ji} Q_\vy\big[\vy_j^{t-\frac{1}{2}} - \underline\vy_j^{t-1}\big], \\ %\label{eq:z_update}\\
\vy_i^{t} =&~ \textstyle \vy_i^{t-\frac{1}{2}} +\gamma_y \big(\vz_i^{t}-\underline\vy_i^{t}\big).\vspace{-0.2cm}
\end{align*}
From the initialization and the updates of $\underline\vy_i^{t}$ and $\vz_i^{t}$, 
%\eqref{eq:alg3_2} and \eqref{eq:z_update}, 
it always holds that
$\vz_i^{t}=\sum_{j=1}^n \W_{ji} \underline\vy_i^{t}$.
The model communication can be done efficiently in the same way. %similar. 


The compression operators $Q_\vx$ and $Q_\vy$ in Algorithm \ref{alg:CDProxSGT} can be different, but we assume that they both satisfy the following assumption. %\YX{Do we need $\alpha < 1$.}
\begin{assumption} \label{assu:compressor}
There exists $\alpha \in [0,1)$ such that  
$$\bbE[\|\vx-Q[\vx]\|^2]\leq \alpha^2 \|\vx\|^2, \forall\, \vx\in\bbR^d,$$ 
for both $Q=Q_\vx$ and $Q=Q_\vy$.
\end{assumption}
% \JC{Is the above assumption standard? If yes, indicate so. If not, discuss it.}
The assumption on compression operators is standard and also made in \cite{koloskova2019decentralized-b,koloskova2019decentralized,zhao2022beer}. It is satisfied by the sparsification, such as Random-$k$ \cite{stich2018sparsified} and Top-$k$ \cite{aji2017sparse}. It can also be satisfied by rescaled quantizations.  For example, QSGD \cite{alistarh2017qsgd} compresses $\vx\in \bbR^d$ by $Q_{sqgd}(\vx) = \frac{\sign(\vx)\|\vx\|}{s} \lfloor s \frac{|\vx|}{\|\vx\|} + \xi \rfloor
$
where $\xi$ is uniformly distributed on $[0,1]^d$, $s$ is the parameter about compression level. Then $Q(\vx)= \frac{1}{\tau} Q_{sqgd} (\vx)$ with $\tau=(1+\min\{d/s^2, \sqrt{d}/s\})$ satisfies Assumption \ref{assu:compressor} with $\alpha^2=1-\frac{1}{\tau}$. More examples can be found in \cite{koloskova2019decentralized}.

Below, we make a couple of remarks to discuss the relations between Algorithm \ref{alg:DProxSGT} and Algorithm \ref{alg:CDProxSGT}.

% \YX{After Algorithm 2, mention that with some special choice of parameters, it will reduce to Algorithm 1. However, we will analyze them separately because ... Also, emphasize that both algorithms are new for the considered problems and have not been studied in the literature.}
\begin{remark}
When $Q_\vx$ and $Q_\vy$ are both identity operators, i.e., $Q_\vx[\vx] = \vx, Q_\vy[\vy] = \vy$, and $\gamma_x=\gamma_y=1$, in Algorithm \ref{alg:CDProxSGT}, CDProxSGT will reduce to DProxSGT. Hence, the latter can be viewed as a special case of the former. However, we will analyze them separately. Although the big-batch training method ProxGT-SA in \cite{xin2021stochastic} shares a similar update as the proposed DProxSGT, our analysis will be completely different and new, as we need only $\mathcal{O}(1)$ samples in each iteration in order to achieve better generalization performance. The analysis of CDProxSGT will be built on that of DProxSGT by carefully controlling the variance error of stochastic gradients and the consensus error, as well as the additional compression error. %Although DProxSGT is similar to ProxGT-SA \cite{xin2021stochastic},  we do not need take $\mathcal{O}(\frac{1}{\epsilon^2})$ samples but only $\mathcal{O}(1)$ samples in each iteration. 
%Thus both DProxSGT and CDProxSGT are new for the considered problems and have not been studied in the literature.
\end{remark}


 

 
% \begin{remark}
% In Algorithms \ref{alg:DProxSGT} and \ref{alg:CDProxSGT}, we use the matrix notation. With $n$ workers,  $\X^t\in \bbR^{d\times n}$ and $\Y^t\in \bbR^{d\times n}$ are column concatenation of $n$ local variable $\vx_i^t\in\bbR^{d}$ and $\vy_i^t\in\bbR^{d}$. $\overline\X^t\in \bbR^{d\times n}$ and $\overline\Y^t\in \bbR^{d\times n}$ are column concatenation of $\overline\vx_i^t\in\bbR^{d}$ and $\overline\vy_i^t\in\bbR^{d}$.
% $\nabla \bF^t\in \bbR^{d\times n}$ are column concatenation of $n$  stochastic gradient $\nabla F_i(\vx_i^t,\xi_i^t)\in\bbR^{d}$.  
% In \eqref{eq:x_half_update}, $\prox_{\eta r}$ is applied  to the column concatenated matrix $\X^t - \eta \Y^{t}$, which means applying it to each column separately, i.e.,  \eqref{eq:x_half_update} euqals to $\vx^{t+\frac{1}{2}}_i = \prox_{\eta r}(\vx^t_i-\eta\vy_i^t)$ for $i=1,2,\ldots, n$.
% \end{remark}

 

\begin{remark}
When $Q_\vy$ and $Q_\vx$ are identity operators, $\underline\vy_i^{t} = \vy_i^{t-\frac{1}{2}}$ and $\underline\vx_i^{t+1} = \vx_i^{t+\frac{1}{2}}$ for each $i\in\hN$. Hence, in the compression case, $\underline\vy_i^{t}$ and $\underline\vx_i^{t+1}$ can be viewed as estimates of  $\vy_i^{t-\frac{1}{2}}$ and $\vx_i^{t+\frac{1}{2}}$. %Note $\underline\Y^{t}$ and $\underline\X^{t}$  estimate $\Y^{t-\frac{1}{2}}$ and $\X^{t-\frac{1}{2}}$, respectively. 
In addition, in a matrix format, we have from \eqref{eq:alg3_3} and \eqref{eq:alg3_6} that
 \begin{align} 
    \Y^{t+1} %=&~ \Y^{t+\frac{1}{2}} + \gamma_y \underline\Y^{t+1}(\W-\I) \nonumber \\
   % =&~ \Y^{t+\frac{1}{2}}\big(\gamma_y \W + (1-\gamma_y)\I\big) + \gamma_y\big(\underline\Y^{t+1}-\Y^{t+\frac{1}{2}}\big)(\W-\I) \nonumber \\
     =&~ \Y^{t+\frac{1}{2}}\widehat\W_y + \gamma_y\big(\underline\Y^{t+1}-\Y^{t+\frac{1}{2}}\big)(\W-\I), \label{eq:Y_hatW}\\
    \X^{t+1} %=&~ \X^{t+\frac{1}{2}} + \gamma_x \underline\X^{t+1}(\W-\I) \nonumber \\
   % =&~ \X^{t+\frac{1}{2}}\big(\gamma_x \W + (1-\gamma_x)\I\big) + \gamma_x\big(\underline\X^{t+1}-\X^{t+\frac{1}{2}}\big)(\W-\I) \nonumber \\
    =&~ \X^{t+\frac{1}{2}}\widehat\W_x + \gamma_x(\underline\X^{t+1}-\X^{t+\frac{1}{2}})(\W-\I), \label{eq:compX_hatW}
\end{align}
where 
$\widehat\W_y = \gamma_y \W + (1-\gamma_y)\I,\ \widehat\W_x = \gamma_x \W + (1-\gamma_x)\I.$
When $\W$ satisfies the conditions (i)-(iii) in Assumption~\ref{assu:mix_matrix}, it can be easily shown that $\widehat\W_y$ and $\widehat\W_x$ also satisfy all three conditions. Indeed, we have
$$\widehat\rho_x \triangleq \|\widehat\W_x - \J\|_2 < 1,\quad 
\widehat\rho_y \triangleq \|\widehat\W_y - \J\|_2 < 1.$$
Thus we can view $\Y^{t+1}$ and $\X^{t+1}$ as the results of $\Y^{t+\frac{1}{2}}$ and $\X^{t+\frac{1}{2}}$ by one round of neighbor communication with mixing matrices $\widehat{\W}_y$ and $\widehat{\W}_x$, and the addition of the estimation error $\underline\Y^{t+1}-\Y^{t+\frac{1}{2}}$ and $\underline\X^{t+1}-\X^{t+\frac{1}{2}}$ after one round of neighbor communication.
\end{remark}
%
%\begin{remark}
%In \eqref{eq:Y_hatW} and \eqref{eq:compX_hatW}, $\widehat\W_y$ and $\widehat\W_x$ are two mixing matrices. Define 
% 
%\end{remark}

 

% \YX{Let's put two algorithms in one section and then convergence results with discussions/explanation on the key analysis steps in another section. State the assumptions on the stochastic gradients and compression operators in the beginning of the analysis section or after giving the algorithms.}




 




 

% In section \ref{sec:DProxSGT}, we introduce the decentralized proximal stochastic gradient decent method with gradient tracking (DProxSGT). Then in section \ref{sec:CDProxSGT}, we propose the compressed method by compressing both models and gradients in DProxSGT and name the new method as CDProxSGT.


==> Decentralized_nonconvex_nonsmooth_ arXiv/analysis.tex <==

\section{Convergence Analysis}

% \YX{Define the Moreau envelope in the analysis section and explain why it can be used as a valid stationarity measure.}
In this section, we analyze the convergence of the algorithms proposed in section~\ref{sec:alg}. Nonconvexity of the problem and stochasticity of the algorithms both raise difficulty on the analysis. In addition, the coexistence of the nonsmooth regularizer $r(\cdot)$ causes more significant challenges.  
To address these challenges, we employ a tool of the so-called Moreau envelope \cite{MR201952}, which has been commonly used for analyzing methods on solving nonsmooth weakly-convex problems.

\begin{definition}[Moreau envelope] Let $\psi$ be an $L$-weakly convex function, i.e., $\psi(\cdot) + \frac{L}{2}\|\cdot\|^2$ is convex. For $\lambda\in(0,\frac{1}{L})$, the Moreau envelope of $\psi$ is defined as
\vspace{-0.2cm}
 \begin{equation*} 
\psi_\lambda(\vx) = \min_\vy \textstyle \left\{\psi(\vy) + \frac{1}{2\lambda}\|\vy-\vx\|^2\right\},  \vspace{-0.2cm}
\end{equation*} 
and the unique minimizer is denoted as
\vspace{-0.2cm}
\begin{equation*}
 \prox_{\lambda \psi}(\vx)= \argmin_{\vy} \textstyle \left\{\psi(\vy)+\frac{1}{2\lambda} \|\vy-\vx\|^2\right\}.\vspace{-0.2cm}
 \end{equation*} 
\end{definition}


%\begin{remark} \label{property:prox}
% When $\lambda \in (0, \frac{1}{L})$, $\phi(\vy) + \frac{1}{2\lambda}\|\vy-\vx\|^2$ is strongly convex with respect to $\vy$ and the minimizer in the Moreau envelope is unique. Denote the minimizer as 
% \begin{align*}
% \prox_{\lambda \phi}(\vx):= \argmin_{\vy} \phi(\vy)+\frac{1}{2\lambda} \|\vy-\vx\|^2.
% \end{align*}
% Furthermore,  we have $\widehat{\vx}=\prox_{\lambda \phi}(\vx)$ if and only if 
% $0 \in \partial \phi(\widehat\vx) + \frac{1}{\lambda}(\widehat\vx-\vx)$.
%\end{remark}

%In the problem \eqref{eq:problem_original}, $\phi$ is nonsmooth, but its Moreau envelope $\phi_\lambda$ is smooth for any $\lambda\in (0, \frac{1}{L})$, because $\phi$ is $L$-weakly convex. In addition, the gradient norm $\|\nabla \phi_\lambda(\vx)\|$ can be used as a valid measure of stationarity violation at $\vx$ for $\phi$, as shown in 
The Moreau envelope $\psi_\lambda$ has nice properties.
The result below can be found in  
  \cite{davis2019stochastic, nazari2020adaptive, xu2022distributed-SsGM}.
 % \cite{davis2019stochastic}, Lemma 8 in \cite{nazari2020adaptive}, Lemma 2.4 in  \cite{xu2022distributed-SsGM}. \YX{The credit for this result should be given to an earlier paper. And this does not sound a lemma but a discussion.}
 \begin{lemma}\label{lem:xhat_x}
 For any function $\psi$, if it is $L$-weakly convex, then for any $\lambda \in (0, \frac{1}{L})$,  the Moreau envelope $\psi_\lambda$ is smooth with gradient given by 
$\nabla \psi_\lambda (\vx) = \lambda^{-1} (\vx-\widehat\vx),$
 where $\widehat\vx=\prox_{\lambda\psi}(\vx)$. 
Moreover, \vspace{-0.2cm}
\[
\|\vx-\widehat\vx\|=\lambda\|\nabla \psi_\lambda(\vx)\|, \quad %\phi(\widehat\vx)\leq\phi(\vx), \quad 
\dist(\0, \partial \psi(\widehat \vx))\leq \|\nabla \psi_\lambda(\vx)\|.\vspace{-0.2cm}
\]
\end{lemma}

Lemma~\ref{lem:xhat_x}  implies that if $\|\nabla \psi_\lambda(\vx)\|$ is small, then $\widehat\vx$ is a near-stationary point of $\psi$ and $\vx$ is close to $\widehat\vx$. Hence, $\|\nabla \psi_\lambda(\vx)\|$ can be used as a valid measure of stationarity violation at $\vx$ for $\psi$. Based on this observation, we define the $\epsilon$-stationary solution below for the decentralized problem \eqref{eq:decentralized_problem}.

%Let $\widehat{\vx}=\prox_{\lambda \phi}(\vx)$. Then it holds \cite{?} $\nabla \phi_\lambda = \frac{1}{\lambda}(\vx-\widehat\vx)$.
% From the optimality condition of $\widehat\vx$, one has 
%\[
%\textstyle
%\0\in \partial \phi(\widehat\vx) + \frac{1}{\lambda}(\widehat\vx-\vx) \mbox{ i.e. } \dist(\0, \partial \phi(\widehat\vx)) \leq \frac{1}{\lambda}\|\widehat\vx-\vx\|.
%\]
%Therefor, if $\frac{1}{\lambda}\|\widehat\vx-\vx\|\leq \epsilon$, then $\widehat\vx$ is $\epsilon$-stationary and $\vx$ is close to the $\epsilon$-stationary point  $\widehat\vx$.

% \YX{Give the definition of the $\epsilon$-solution we aim at.}
\begin{definition}[Expected $\epsilon$-stationary solution]\label{def:eps-sol} Let $\epsilon > 0$. A point $\X = [\vx_1, \ldots, \vx_n]$ is called an expected $\epsilon$-stationary solution of \eqref{eq:decentralized_problem} if for a constant $\lambda\in (0, \frac{1}{L})$,
    \vspace{-0.1cm}
\begin{equation*}
    \textstyle\frac{1}{n} \bbE\left[\sum_{i=1}^n \|\nabla \phi_\lambda(\vx_i)\|^2 + L^2 \|\X_\perp\|^2\right] \leq \epsilon^2.
%where $\widehat\X = [\widehat\vx_1, \ldots, \widehat\vx_n]$ with $\widehat{\vx}_i \triangleq \prox_{\lambda \phi}(\vx_i), \forall\, i\in\hN$.
    \vspace{-0.1cm}
\end{equation*}
\end{definition}  

In the definition above, $L^2$ before the consensus error term $\|\X_\perp\|^2$ is to balance the two terms. This scaling scheme has also been used in existing works such as \cite{xin2021stochastic,mancino2022proximal,DBLP:journals/corr/abs-2202-00255} . From the definition, we see that if $\X$ is an expected $\epsilon$-stationary solution of \eqref{eq:decentralized_problem}, then each local solution $\vx_i$ will be a near-stationary solution of $\phi$ and in addition, these local solutions are all close to each other, namely, they are near consensus.

% \YX{Revise the complexity results to give an expected $\epsilon$-stationary solution. Among the $T$ generated iterates, pick an iterate $\X^\tau$ uniformly at random.}

Below we first state the convergence results of the non-compressed method DProxSGT %in 
%Algorithm~\ref{alg:DProxSGT} 
and then the compressed one CDProxSGT. %in Algorithm~\ref{alg:CDProxSGT}. 
All the proofs are given in the appendix.
 
\begin{theorem}[Convergence rate of DProxSGT]\label{thm:sec2}
Under Assumptions \ref{assu:prob} -- \ref{assu:stoc_grad}, let $\{\X^t\}$ be generated from $\mathrm{DProxSGT}$ in Algorithm~\ref{alg:DProxSGT} with $\vx_i^0 = \vx^0, \forall\, i \in \hN$. Let  $\lambda = \min\big\{\frac{1}{4 L}, \frac{1}{96\rho L}\big\}$ and $\eta\leq  \min\big\{\frac{1}{4 L},\frac{(1-\rho^2)^4}{96\rho  L}\big\}$. 
Select $\tau$ from $\{0, 1, \ldots, T-1\}$ uniformly at random.
Then 
\vspace{-0.1cm}
\begin{equation*}%\label{eq:them_DProxSGT}
\begin{aligned} 
   &~ \textstyle \frac{1}{n} \bbE\left[\sum_{i=1}^n \|\nabla\phi_\lambda(\vx_i^\tau)\|^2 +\frac{4}{\lambda \eta} \|\X^\tau_\perp\|^2\right]  \\
   \leq &~ \textstyle \frac{8\left( \phi_\lambda(\vx^0) - \phi_\lambda^*\right)}{ \eta T}  + \frac{4616 \eta}{\lambda(1-\rho^2)^3} \sigma^2 \textstyle  + \frac{768\eta  \bbE\left[ \|\nabla \bF^0(\I-\J)\|^2\right]}{n\lambda T(1-\rho^2)^3},
\end{aligned}
\vspace{-0.1cm}
\end{equation*}
where $\phi_\lambda^* = \min_{\vx} \phi_\lambda(\vx)> -\infty$. %\YX{The lower bound cannot be $-\infty$.}
\end{theorem}
 

By Theorem~\ref{thm:sec2}, we obtain a complexity result as follows.

% In order to have an expected $\epsilon$-stationary point of \eqref{eq:decentralized_problem}, we need the right side of \eqref{eq:them_DProxSGT} is less than $\epsilon^2$. 
% \begin{gather*}
%     \frac{4616 \eta}{\lambda(1-\rho^2)^3} \sigma^2 \leq  \frac{\epsilon^2}{2},\\
%     \textstyle  \frac{8\left( \phi_\lambda(\vx^0) - \phi_\lambda^*\right)}{ \eta T} + \frac{768\eta  \bbE\left[ \|\nabla \bF^0(\I-\J)\|^2\right]}{n\lambda T(1-\rho^2)^3} \leq \frac{\epsilon^2}{2}.
% \end{gather*}
 
\begin{corollary}[Iteration complexity]
Under the assumptions of Theorem~\ref{thm:sec2}, 
for a given $\epsilon>0$, take $ \eta = \min\{\frac{1}{4 L},\frac{(1-\rho^2)^4}{96\rho  L}, \frac{ \lambda(1-\rho^2)^3 \epsilon^2}{9232\sigma^2}\}$. Then $\mathrm{DProxSGT}$ can find an expected $\epsilon$-stationary point of \eqref{eq:decentralized_problem}  when $T \geq  T_\epsilon = \left\lceil \frac{16\left( \phi_\lambda(\vx^0) - \phi_\lambda^*\right)}{ \eta \epsilon^2 } + \frac{1536\eta  \bbE\left[ \|\nabla \bF^0(\I-\J)\|^2\right]}{n\lambda (1-\rho^2)^3 \epsilon^2} \right\rceil$.  
\end{corollary}
 
% \YX{Check how the dependence on $(1-\rho)$ compares to the paper in IEEE about a decentralized subgradient method.}
 
\begin{remark} \label{remark:DProxSGT}
When %the given tolerance 
$\epsilon$ is small enough, $\eta$ will take $\frac{ \lambda(1-\rho^2)^3 \epsilon^2}{9232\sigma^2}$, and $T_\epsilon$ will be dominated by the first term. 
% $  \frac{16\left( \phi_\lambda(\vx^0) - \phi_\lambda^*\right) 9232\sigma^2}{  \lambda(1-\rho^2)^3 \epsilon^4}$
In this case, DProxSGT can find an expected $\epsilon$-stationary solution of \eqref{eq:decentralized_problem} in $O\Big( \frac{\sigma^2\left( \phi_\lambda(\vx^0) - \phi_\lambda^*\right) }{\lambda(1-\rho^2)^3 \epsilon^4}\Big)$ iterations, leading to the same number of stochastic gradient samples %at each node 
and communication rounds. Our sample complexity is optimal in terms of the dependence on $\epsilon$ under the smoothness condition in Assumption~\ref{assu:prob}, as it matches with the lower bound in \cite{arjevani2022lower}. However, the dependence on $1-\rho$ may not be optimal because of our possibly loose analysis, as the \emph{deterministic} method with single communication per update in \cite{scutari2019distributed} for nonconvex nonsmooth problems has a dependence $(1-\rho)^2$ on the graph topology. %Hence, our  and can possibly be further reduced. 
\end{remark}


 

 

% \subsection{Compressed Decentralized proximal stochastic gradient decent method with gradient tracking (CDProxSGT)}  \label{sec:CDProxSGT}
 
% \YX{Do similar revisions to the results of CDProxSGT. Then revise the proofs accordingly.}
\begin{theorem}[Convergence rate of CDProxSGT] \label{thm:sect3thm}
 Under Assumptions \ref{assu:prob} through \ref{assu:compressor},
 let $\{\X^t\}$ be generated from $\mathrm{CDProxSGT}$ in Algorithm \ref{alg:CDProxSGT} with
 $\vx_i^0 = \vx^0, \forall\, i \in \hN$. Let $\lambda = \min \big\{\frac{1}{4 L}, \frac{ (1-\alpha^2)^2}{9 L+41280}\big\}$, and suppose
\vspace{-0.1cm}
\begin{gather*}
 \eta \leq~ \min\left\{ \textstyle \lambda, %\frac{1-\widehat\rho^2_y}{8\sqrt{5} L}, 
 \frac{(1-\alpha^2)^2(1-\widehat\rho^2_x)^2(1-\widehat\rho^2_y)^2}{18830\max\{1, L\}}\right\}, \\
\gamma_x\leq~ \min\left\{ \textstyle %\frac{2\sqrt{3}-3}{6\alpha},
%\frac{ 1-\widehat\rho_x^2}{60\alpha},   
\frac{1-\alpha^2}{25}, \frac{\eta}{\alpha}%,  \frac{1}{6\alpha}
\right\}, \quad 
 \gamma_y\leq ~   \textstyle 
 \frac{(1-\alpha^2)(1-\widehat\rho^2_x)(1-\widehat\rho^2_y)}{317}.
\end{gather*}
\vspace{-0.1cm}
Select $\tau$ from $\{0, 1, \ldots, T-1\}$ uniformly at random.
Then 
\vspace{-0.1cm}
\begin{equation*}%\label{eq:them_CDProxSGT}
    \begin{aligned}
   &~ \textstyle \frac{1}{n} \bbE\left[\sum_{i=1}^n \|\nabla\phi_\lambda(\vx_i^\tau)\|^2 +\frac{4}{\lambda \eta} \|\X^\tau_\perp\|^2\right]   \\
   \leq &~\textstyle \frac{8\left(\phi_\lambda(\vx^0) - \phi_\lambda^*\right)}{\eta T}  
     +\frac{(50096n+48)\eta \sigma^2}{n\lambda(1-\widehat\rho^2_x)^2(1-\widehat\rho^2_y)} +   \frac{4176 \eta \bbE\left[ \|\nabla \bF^0\|^2\right] }{n\lambda T (1-\widehat\rho^2_x)^2(1-\widehat\rho^2_y)},
\end{aligned}
\vspace{-0.1cm}
\end{equation*}
where $\phi_\lambda^* = \min_{\vx} \phi_\lambda(\vx)> -\infty$. %\YX{Cannot be $-\infty$.}
\end{theorem}
% \begin{remark}
% When the conditions of Theorem \ref{thm:sect3thm} hold, the consensus error of $\X$ satisfies
% \begin{align*}
%    &~\frac{1}{nT}\sum_{t=0}^{T-1} \bbE\big[\|\X^t_\perp\|^2\big]\leq   \textstyle  \frac{1044 \eta^2 \bbE\left[ \|\nabla \bF^0\|^2\right] }{n T (1-\widehat\rho^2_x)^2(1-\widehat\rho^2_y)} \\
%    &~  \textstyle  +\frac{2\lambda\left(\Phi^0 -\Phi^{T}\right)}{n T} +\frac{(12524 n + 12)\eta^2 \sigma^2}{n(1-\widehat\rho^2_x)^2(1-\widehat\rho^2_y)^2}.
% \end{align*}
% \end{remark}

By Theorem~\ref{thm:sect3thm}, we have the complexity result as follows.

\begin{corollary}[Iteration complexity]
Under the assumptions of Theorem \ref{thm:sect3thm}, for a given $\epsilon>0$, take 
\begin{gather*}
    \eta = \textstyle \min \left\{\frac{1}{4 L}, \frac{ (1-\alpha^2)^2}{9 L+41280}, \frac{(1-\alpha^2)^2(1-\widehat\rho^2_x)^2(1-\widehat\rho^2_y)^2}{18830\max\{1, L\}}\right.,\\ \textstyle  \left. \frac{n\lambda(1-\widehat\rho^2_x)^2(1-\widehat\rho^2_y)\epsilon^2}{2(50096n+48) \sigma^2}\right\}, \\
%\end{gather*}
%\begin{gather*} 
   \textstyle  \gamma_x = \min\left\{ \textstyle  
\frac{1-\alpha^2}{25}, \frac{\eta}{\alpha}\right\}, \quad
 \gamma_y =  \frac{(1-\alpha^2)(1-\widehat\rho^2_x)(1-\widehat\rho^2_y)}{317}.
\end{gather*}
Then $\mathrm{CDProxSGT}$ can find an expected $\epsilon$-stationary point of \eqref{eq:decentralized_problem} when  $T\geq T_\epsilon^c$ where 
\begin{align*} 
    T_\epsilon^c = \textstyle \left\lceil\frac{16\left(\phi_\lambda(\vx^0) - \phi_\lambda^*\right)}{\eta \epsilon^2}  +   \frac{8352 \eta \bbE\left[ \|\nabla \bF^0\|^2\right] }{n\lambda (1-\widehat\rho^2_x)^2(1-\widehat\rho^2_y)\epsilon^2} \right\rceil.
\end{align*}
 

%  \begin{gather*}
% T \geq  \textstyle  \frac{n\left(\phi_\lambda(\vx^0) - \phi_\lambda^*\right)(1-\widehat\rho^2_x)^2(1-\widehat\rho^2_y)^2}{(6262 n + 6) \sigma^2 \min\left\{ \textstyle \lambda,  
%  \frac{(1-\alpha^2)^4(1-\widehat\rho^2_x)^2(1-\widehat\rho^2_y)^2}{18830^2\lambda\max\{1, L^2\}}\right\}},\\
% \textstyle \eta = \sqrt{ \frac{2\lambda n\left(\phi_\lambda(\vx^0) - \phi_\lambda^*\right)}{(12524 n + 12)T }} \frac{(1-\widehat\rho^2_x)(1-\widehat\rho^2_y)}{\sigma},\\
% \gamma_x\leq \min\{ \textstyle    
% \frac{1-\alpha^2}{25}, \frac{\eta}{\alpha},  \frac{1}{6\alpha}\},\\
% \gamma_y\leq \min\left\{ \textstyle \frac{\sqrt{1-\widehat\rho^2_y}}{12\alpha}, 
%  \frac{(1-\alpha^2)(1-\widehat\rho^2_x)(1-\widehat\rho^2_y)}{317}\right\}.
% \end{gather*}
% Then 
% \begin{align*}
%    &~ 
%    \textstyle \frac{1}{n} \bbE\left[\sum_{i=1}^n \|\nabla\phi_\lambda(\vx_i^\tau)\|^2 +\frac{4}{\lambda \eta} \|\X^\tau_\perp\|^2\right] 
%   \\
%    \leq &~ \textstyle\sqrt{ \frac{ \phi_\lambda(\vx^0) - \phi_\lambda^* }{ \lambda T  (1-\widehat\rho^2_x)^2 }}\Big(  \frac{1267 \sigma}{(1-\widehat\rho^2_y)}    +  \frac{53 \bbE\left[ \|\nabla \bF^0\|^2\right] }{n T \sigma }\Big).
% \end{align*}
% And
% \begin{align*}
%    &~\frac{1}{nT}\sum_{t=0}^{T-1} \bbE\big[\|\X^t_\perp\|^2\big]\leq   \textstyle \frac{\lambda\left(\Phi^0 -\Phi^{T}\right)}{n T} \Big( 4 +\frac{   (1-\widehat\rho^2_y)   \bbE\left[ \|\nabla \bF^0\|^2\right] }{7n  T  \sigma^2}\Big).
% \end{align*}

% Hence, given $\epsilon > 0$, $\mathrm{CDProxSGT}$ can find an expected $\epsilon$-stationary point of \eqref{eq:decentralized_problem} in at most $T_\epsilon^c$ iterations, where
% \begin{align*} 
%     T_\epsilon^c = &~\left\lceil  \max \bigg\{  \frac{1267^2\sigma^2 \left(\phi_\lambda(\vx^0) - \phi_\lambda^* \right) }{ \lambda   (1-\widehat\rho^2_x)^2 (1-\widehat\rho^2_y)^2  \epsilon^4 }\right., \\
%      &~\left.\sqrt[3]{\frac{ 53^2\left(\phi_\lambda(\vx^0) - \phi_\lambda^* \right)  \bbE\left[ \|\nabla \bF^0\|^2\right]^2}{ \lambda n^2  (1-\widehat\rho^2_x)^2\sigma^2 \epsilon^4}} \bigg\}\right\rceil,
% \end{align*}
% provided that 
% \[
%     T_\epsilon^{c}\geq \textstyle  \frac{n\left(\phi_\lambda(\vx^0) - \phi_\lambda^*\right)(1-\widehat\rho^2_x)^2(1-\widehat\rho^2_y)^2}{(6262 n + 6) \sigma^2 \min\left\{ \textstyle \lambda,  
%     \frac{(1-\alpha^2)^4(1-\widehat\rho^2_x)^2(1-\widehat\rho^2_y)^2}{18830^2\lambda\max\{1, L^2\}}\right\}}.
%  \]
\end{corollary}

\begin{remark}
When the given tolerance $\epsilon$ is small enough,
$\eta$ will take $\frac{n\lambda(1-\widehat\rho^2_x)^2(1-\widehat\rho^2_y)\epsilon^2}{2(50096n+48) \sigma^2}$ and $T_\epsilon^c$ will be dominated by the first term. In this case, similar to DProxSGT in Remark \ref{remark:DProxSGT}, CDProxSGT can find an expected $\epsilon$-stationary solution of \eqref{eq:decentralized_problem} in $O\Big( \frac{\sigma^2\left( \phi_\lambda(\vx^0) - \phi_\lambda^*\right) }{ \lambda(1-\widehat\rho^2_x)^2(1-\widehat\rho^2_y) \epsilon^4}\Big)$ iterations. %leading to the same number of stochastic gradient samples at each node and communication rounds.
\end{remark} 

==> Decentralized_nonconvex_nonsmooth_ arXiv/experiments.tex <==
\section{Numerical Experiments}\label{sec:numerical_experiments}
In this section, we test the proposed algorithms on training two neural network models, in order to demonstrate their better generalization over momentum variance-reduction methods and large-batch training methods and to demonstrate the success of handling heterogeneous data even when only compressed model parameter and gradient information are communicated among workers.
One neural network that we test is LeNet5  \cite{lecun1989backpropagation} on the FashionMNIST dataset \cite{xiao2017fashion}, and the other is FixupResNet20 \cite{zhang2019fixup} on Cifar10 \cite{krizhevsky2009learning}. 
% \YX{The two data sets are well-known. We may not need to mention the number of samples and size, but just mention the number of classes, because they will be distributed based on the class.} 
% Fashion-MNIST includes 60,000 training samples and 10,000 test samples with each sample as a 28x28 grayscale image. 
% Cifar10 includes 50000 training samples and 10000 test samples with each sample as a 32x32 colour image. 

Our experiments are representative to show the practical performance of our methods. Among several closely-related works,  \cite{xin2021stochastic} includes no experiments, and \cite{mancino2022proximal,zhao2022beer} only tests on tabular data and MNIST. \cite{koloskova2019decentralized-b} tests its method on Cifar10 but needs %with distinct data between nodes during the training, but the data on all nodes has 
similar data distribution on all workers 
for good performance.
%Although with similar-scale as MNIST, 
FashionMNIST has a similar scale as MNIST but poses a more challenging classification task \cite{xiao2017fashion}. 
% \YX{Mention the challenges of FashionMNIST. Otherwise reviewers would think it is the same as MNIST.}.  
Cifar10 is more complex, and FixupResNet20 has more layers than LeNet5.  
 


% \PYB{We may need to comment that these tasks and models are of similar-scale as the experiments shown in other related works; o.w., reviewers may simply ask us to run on more datasets and models. We also need to emphasize these experiments are representative to validate the theoretical insights that we proved}

% \YX{This paragraph is redundant. The description is also made in the next two subsections.} We first compare DProxSGT with AllReduce\footnote{In AllReduce, model parameters (or equivalently the stochastic gradients) are averaged among all nodes in each iteration. We see AllReduce as a baseline.}, DEEPSTORM\footnote{For DEEPSTORM, we implement the verison of DEEPSTORM v2 in \cite{mancino2022proximal}.} \cite{mancino2022proximal} and ProxGT-SA \cite{xin2021stochastic} by training the models with the regularization $r(\vx) = \mu\|\vx\|_1$ in Section %\PYB{subsection $\rightarrow$ Section} 
% \ref{subsect:RegL1}. 
% Then we compare the compressed CDProxSGT with AllReduce, DProxSGT, Choco-SGD \cite{koloskova2019decentralized,koloskova2019decentralized-b} and BEER \cite{zhao2022beer} by training the models with $r(\vx)=0$ in Section \ref{subsect:compress}.
 
All the compared algorithms are implemented in Python with Pytorch %for tensor computing 
and MPI4PY (for distributed computing). %the communication between different nodes, and 
They run on a Dell workstation with %32 CPU cores, 64 GB memory, and 
two Quadro RTX 5000 GPUs. We use the 2 GPUs as 5 workers, which communicate over a ring-structured network (so each worker can only communicate with two neighbors). Uniform weight is used, i.e., $W_{ji} = \frac{1}{3}$ for each pair of connected workers $i$ and $j$. %We test our algorithms on extremely heterogeneous data, i.e., the samples are divided to the nodes by labels. 
Both FashionMNIST and Cifar10 have 10 classes. We distribute each data onto the 5 workers based on the class labels, namely, each worker holds 2 classes of data points, and thus the data are heterogeneous across the workers. %, i.e., each sample is labeled by one of $0,1,\ldots,9$. 
%The 2 GPUs cannot run 10 processes due to the limited memory of GPUs. We evaluates on 5 processes i.e. 5 nodes.  The 5 nodes are connected in a ring and the mixing matrix is set by $W_{ji} = \frac{1}{3}$ when $ (|i-j|  \mod 4) \leq 1$ otherwise $0$ for all $i, j\in\{0,1,2,3,4\}$. We divide the whole training dataset into five heterogeneous subsets. Specifically, each node has a subset with samples of two classes, i.e., for $i =0,1,2,3,4$, node $i$ has the samples with classes $i$ and $9-i$. 

For all methods, we report their objective values on training data, prediction accuracy on testing data, and consensus errors at each epoch. 
To save time, the objective values are computed as the average of the losses that are evaluated during the training process (i.e., on the sampled data instead of the whole training data) plus the regularizer per epoch. 
% \YX{Do you mean the objective values are the averages over all iterates per epoch?}
For the testing accuracy, we first compute the accuracy on the whole testing data for each worker by using its own model parameter and then take the average. %by the local models $\{\vx_i\}_{i\in\hN}$ after each epoch. And 
The consensus error is simply $\|\X_\perp\|^2$. %for $\{\vx_i\}_{i\in\hN}$ 
%after each epoch. %Notice that the AllReduce method is a centralized method The consensus error from  is always $0$ and thus is not shown in the figures of results plotted by ``semilogy".

\subsection{Sparse Neural Network Training} \label{subsect:RegL1}
In this subsection, we test the non-compressed method DProxSGT and compare it with AllReduce (that is a centralized method and used as a baseline), DEEPSTORM\footnote{For DEEPSTORM, we implement DEEPSTORM v2 in \cite{mancino2022proximal}.} and ProxGT-SA \cite{xin2021stochastic} on solving \eqref{eq:decentralized_problem}, where  $f$ is the loss on the whole training data and $r(\vx) = \mu\|\vx\|_1$ serves as a sparse regularizer that encourages a sparse model. %The $1$-norm regularization pushes the model parameters toward $0$ and becoming sparse.

For training LeNet5 on FashionMNIST, we set $\mu= 10^{-4}$ and run each method to 100 epochs. The learning rate $\eta$ and batchsize are set to $0.01$ and 8 for AllReduce and DProxSGT. 
DEEPSTORM uses the same $\eta$ and batchsize but with a larger initial batchsize 200, 
%an additional 200 samples for the initial gradient estimate, 
and its momentum parameter is tuned to $\beta=0.8$ in order to yield the best performance. %, which is the best among $\{0.2, 0.5, 0.8\}$.
ProxGT-SA is a large-batch training method. %implemented by almost the same as DProxSGT, except it uses a larger 
We set its batchsize to 256 and accordingly apply a larger step size $\eta=0.3$ that is the best among $\{0.1, 0.2, 0.3, 0.4\}$. %$\eta=0.2$ and $0.3$ give similar results and are the best in $\{0.1, 0.2, 0.3, 0.4\}$.

For training FixupResnet20  on Cifar10, we set $\mu= 5 \times 10^{-5}$ and run each method to 500 epochs. %We use $\eta=0.02$ and batchsize=64 for 
The learning rate and batchsize are set to $\eta=0.02$ and 64 for AllReduce, DProxSGT, and DEEPSTORM. The initial batchsize is set to 1600 for DEEPSTORM and the momentum parameter set to $\beta=0.8$. 
%For DEEPSTORM uses $\eta=0.02$ and batchsize=64, with additional 1600 samples for the initial gradient estimate, and the best $\beta=0.8$ is selected from $0.2, 0.5, 0.8$.
ProxGT-SA uses a larger batchsize 512 and a larger stepsize $\eta=0.1$ that gives the best performance among $\{0.05, 0.1, 0.2, 0.3\}$. % $\eta=0.05$ and $0.1$ give similar results and are the best in $\{0.05, 0.1, 0.2, 0.3\}$. 

\begin{figure}[ht] 
\begin{center}  
\includegraphics[width=.9\columnwidth]{./figures/noncompressed} 
\vspace{-0.2cm}
\caption{Results of training sparse neural networks by non-compressed methods with $r(\vx) = \mu \|\vx\|_1$ for the same number of epochs. Left: LeNet5 on FashionMNIST with $\mu=10^{-4}$. Right: FixupResnet20 on Cifar10 with $\mu=5\times 10^{-5}$.}
\label{fig:RegL1}
\end{center} 
\end{figure}

% \begin{figure*}[ht] 
% \begin{center} 
% \includegraphics[width=1.95\columnwidth]{./figures/FMNIST_Lenet5} \\
% \includegraphics[width=1.95\columnwidth]{./figures/Cifar10_fixupresnet}  
% \caption{Results of training sparse neural networks by non-compressed methods with $r(\vx) = \mu \|\vx\|_1$ for the same number of epochs. Top: LeNet5 on FashionMNIST with $\mu=10^{-4}$. Bottom: FixupResnet20 on Cifar10 with $\mu=5\times 10^{-5}$.}
% \label{fig:RegL1}
% \end{center} 
% \end{figure*}

The results for all methods are plotted in Figure \ref{fig:RegL1}. For LeNet5, DProxSGT produces almost the same curves as the centralized training method AllReduce, while on FixupResnet20, DProxSGT even outperforms AllReduce in terms of testing accuracy. This could be because AllReduce aggregates stochastic gradients from all the workers for each update and thus equivalently, it actually uses a larger batchsize. %i.e., updates the models with the batch size of $64\times 5=320$. 
DEEPSTORM performs equally well as our method DProxSGT on training LeNet5. However, it gives lower testing accuracy than DProxSGT and also oscillates significantly more seriously on training the more complex neural network FixupResnet20. This appears to be caused by the momentum variance reduction scheme used in DEEPSTORM.
%The consensus errors from DProxSGT and DEEPSTORM oscillate around the same range. And DEEPSTORM performs almost the same as AllReduce and DProxSGT while training LeNet5, but while training the larger model FixupResnet20, the objective curve is as good as AllReduce but the testing accuracy curvy is lower and has large oscillations. We believe that the lower performance of DEEPSTORM on the testing accuracy is because of the momentum variance reduction schemes. 
In addition, we see that the large-batch training method ProxGT-SA performs much worse than DProxSGT within the same number of epochs (i.e., data pass), especially on training FixupResnet20. %converges much slower and has larger consensus error than the other three methods. For training LeNet5, the objective and testing accuracy curves of ProxGT-SA also arrive plateau after about 60 epochs, but the plateau objective is higher and the plateau testing accuracy is lower than others. For training FixupResnet20,  the objective and testing accuracy curves of ProxGT-SA do not arrive plateau in 500 epochs while the curves of other methods arrive  plateau after about 400 epochs. ProxGT-SA requires a large batch size which means less iterations in the given epochs and a larger best step size. Less iteration and large step size should be the reason why ProxGT-SA  converges slowly and oscillates in a larger range. 
%Thus our proposed DProxSGT performs the best, DEEPSTORM performs well for the small neural network LeNet5 but its generalization on testing data for larger neural network FixupResnet20 lowers down. ProxGT-SA is far from others while training both the two models. 
% \YX{From the observation, state the possible reason that DEEPSTORM and ProxGT-SA gives lower testing accuracy. This will support our motivation of studying the small-batch method without momentum variance reduction.}

\subsection{Neural Network Training by Compressed Methods} \label{subsect:compress}
In this subsection, we compare CDProxSGT with two state-of-the-art compressed training methods: Choco-SGD \cite{koloskova2019decentralized,koloskova2019decentralized-b} and BEER \cite{zhao2022beer}. As Choco-SGD and BEER are studied only for  problems without a regularizer, we set $r(\vx)=0$ in \eqref{eq:decentralized_problem} for the tests. Again, we compare their performance on training LeNet5 and FixupResnet20. %the two neural networks in Section \ref{subsect:RegL1}. 
The two non-compressed methods AllReduce and  DProxSGT are included as baselines.  %In the testing, 
The same compressors are used for CDProxSGT, Choco-SGD, and BEER, when compression is applied. %all the methods when compression is performed.

\begin{figure}[htbp] 
\begin{center} 
\includegraphics[width=.9\columnwidth]{./figures/Compressed}  
\vspace{-0.2cm}
\caption{Results of training neural network models by compressed methods for the same number of epochs.  Left: LeNet5 on FashionMNIST. Right: FixupResnet20 on Cifar10.}
\label{fig:Compress}
\end{center} 
\end{figure} 

We run each method to 100 epochs for training LeNet5 on FashionMNIST. 
The compressors $Q_y$  and $Q_x$ are set to top-$k(0.3)$ \cite{aji2017sparse}, i.e., taking the largest $30\%$ elements of an input vector in absolute values and zeroing out all others. %as $0$, i.e., , and .
We set batchsize to 8 and tune the learning rate $\eta$ to $0.01$ for AllReduce, DProxSGT, CDProxSGT and Choco-SGD, and for CDProxSGT, we set $\gamma_x=\gamma_y=0.5$. 
BEER is a large-batch training method. It uses a larger batchsize 256 and accordingly a larger learning rate $\eta=0.3$, which appears to be the best among $\{0.1, 0.2, 0.3, 0.4\}$. 
% \YX{Mention that the compared methods use the same compressor where compression is performed.}
 
For training FixupResnet20 on the Cifar10 dataset, we run each method to 500 epochs. We take top-$k(0.4)$ \cite{aji2017sparse} as the compressors $Q_y$  and $Q_x$ and set $\gamma_x=\gamma_y=0.8$.
For AllReduce, DProxSGT, CDProxSGT and Choco-SGD, we set their batchsize to 64 and tune the learning rate $\eta$ to $0.02$. For BEER, we use a larger batchsize 512 and a larger learning rate $\eta=0.1$, which is the best among
%$\eta=0.05$ and $0.1$ give similar results and are the best in
$\{0.05, 0.1, 0.2, 0.3\}$. 

The results are shown in Figure \ref{fig:Compress}. 
For both models, CDProxSGT yields almost the same curves of objective values and testing accuracy as its non-compressed counterpart DProxSGT and the centralized non-compressed method AllReduce. This indicates about 70\% saving of communication for the training of LeNet5 and 60\% saving for FixupResnet20 without sacrifying the testing accuracy. %has slightly higher consensus errors than DProxSGT, but CDProxSGT performs almost the same in objective and testing accuracy as DProxSGT and AllReduce. Compared with DProxSGT, CDProxSGT transmit only 30\% and 40\% amount in communication for training LeNet5 and FixupResnet20 respectively but keep the same testing accuracy. 
In comparison, BEER performs significantly worse than the proposed method CDProxSGT within the same number of epochs in terms of all the three measures, especially on training the more complex neural network FixupResnet20, which should be attributed to the use of a larger batch by BEER. Choco-SGD can produce comparable objective values. However, its testing accuracy is much lower than that produced by our method CDProxSGT. %has a large consensus error and converges slower in objective and testing accuracy: BEER has a higher plateau objective and lower plateau testing accuracy in training LeNet5 and does not arrive plateau in 500 epochs while others arrive after about 400 epochs in training FixupResnet20.
%The testing accuracy from Choco-SGD is far from others, although its objective is not the worst one, or even is the best for training LeNet5, and its consensus error is similar to CDProxSGT's. 
This should be because of the data heterogeneity that ChocoSGD cannot handle, while CDProxSGT applies the gradient tracking to successfully address the challenges of data heterogeneity. %, and thus the models on each node converge to the local optimal. 
%The objective is the average of local objectives evaluated at local model, and the testing accuracy is the average of accuracy on whole data evaluated at local models. Thus gradient tracking is essential for training on heterogenous data.   



% \begin{figure*}[htbp] 
% \begin{center} 
% \includegraphics[width=1.95\columnwidth]{./figures/Compress_FMNIST_Lenet5} \\
% \includegraphics[width=1.95\columnwidth]{./figures/Compress_Cifar10_fixupresnet} 
% \caption{Results of training neural network models by compressed methods for the same number of epochs.  Top: LeNet5 on FashionMNIST. Bottom: FixupResnet20 on Cifar10.}
% \label{fig:Compress}
% \end{center} 
% \end{figure*}

% \subsection{The effect of the distributed parallel computing for BNN} 
% For binary neural network (BNN), the weights (and activations) are either 1 or -1 \cite{yang2020proxsgd}.

% The achieve the binary neural network, the loss function is combined with a penalty term for the non-binary weights: 
% \begin{align*}
%     \min_{\vx,\va}&  \frac{1}{m} \sum_{i=1}^m f_i(\vx,\vy_i) + \frac{\mu}{4} \sum_{j=1}^n (a_j(x_j+1)^2+(1-a_j)(x_j-1)^2), \\
%     \mbox{s.t. } & a_j = 0  \mbox{ or } 1, j=1,\ldots, n,
% \end{align*}
% where $\mu$ is a given penality parameter. The binary variable $a_j$ can be interpreted as a switch for weight $x_j$. The integer constraints are relaxed to continuous variable in $[0,1]$. 
% \begin{align*}
%     \min_{\vx,\va}&  \frac{1}{m} \sum_{i=1}^m f_i(\vx,\vy_i) + \frac{\mu}{4} \sum_{j=1}^n (a_j(x_j+1)^2+(1-a_j)(x_j-1)^2), \\
%     \mbox{s.t. } & 0 \leq a_j \leq 1, j=1,\ldots, n.
% \end{align*}
% Try 5 dense linear layers with \red{$tanh$} activation function on MNIST. $\mu = 0.0002$. 

% Compare with one worker case to show the parallel advsntages. 

% Show the percentage of binary parameters.


==> Decentralized_nonconvex_nonsmooth_ arXiv/problem.tex <==
\section{Introduction} 
In this paper, we consider to solve nonconvex stochastic composite problems in a decentralized setting:
 \vspace{-0.1cm}
\begin{equation}\label{eq:problem_original}
 \begin{aligned}
&  \min_{\vx\in\bbR^d} \phi(\vx) = f(\vx) + r(\vx),\\[-0.1cm] 
& \text{with } f(\vx)=\frac{1}{n}\sum_{i=1}^n f_i(\vx), f_i(\vx)\!=\!\bbE_{\xi_i \sim \mathcal{D}_i}[F_i(\vx,\xi_i)].
    \end{aligned}
 \vspace{-0.1cm}   
\end{equation}
% \vspace{-0.1cm}
Here, $\{\mathcal{D}_i\}_{i=1}^n$ are possibly \emph{non-i.i.d data} distributions on $n$ machines/workers that can be viewed as nodes of a connected graph $\hG$, and each $F_i(\cdot, \xi_i)$ can only be accessed by the $i$-th worker. 
We are interested in problems %in the form of \eqref{eq:problem_original} 
that satisfy the following structural assumption. 
%\PYB{Can we change the numbering to Assumption 1, instead of 1.1? (same for other assumptions/theorems/lemmas)}
\begin{assumption}[Problem structure] \label{assu:prob}
%For the problems, 
We assume that 
\vspace{-1.5mm}
\begin{itemize}  
\item[(i)] $r$ is closed convex and possibly nondifferentiable.
\item[(ii)] Each $f_i$ is $L$-smooth in $\dom(r)$, i.e., $\|\nabla f_i(\vx) - \nabla f_i(\vy)\| \le L \|\vx- \vy\|$, for any $\vx, \vy\in\dom(r)$. 
\item[(iii)] $\phi$ is lower bounded, i.e.,  $\phi^* \triangleq \min_\vx \phi(\vx) > -\infty$.
\end{itemize}
\vspace{-2mm}
\end{assumption}

%{\color{blue}SL put the assumptions in the theoretical section. you only need this for the theoretical results rather than introduction of the algorithm. the main contribution is the nonsmooth term. focus on the nonsmooth part here. give some motivating examples, and argue why this is important and practical.}

Let $\hN=\{1, 2, \ldots, n\}$ be the set of nodes of $\hG$ and $\hE$ the set of edges. %and can only communicate along the edges $\hE$. Let 
For each $i\in\hN$, denote $\hN_i$ as the neighbors of worker $i$ and itself, i.e., $\hN_i = \{j: (i,j) \in \hE\}\cup \{i\}$. Every worker can only communicate with its neighbors. To solve \eqref{eq:problem_original} collaboratively, each worker $i$ maintains a copy, denoted as $\vx_i$, of the variable $\vx$. With these notations, 
 % 
%Define $\phi_i(\vx) = f_i(\vx) + r(\vx)$. We have  $\phi =\frac{1}{n} \sum_{i=1}^n \phi_i(\vx)$. Let every worker has  Then 
\eqref{eq:problem_original} can be formulated equivalently to %the following distributed optimization problem over the graph $\hG$:
\vspace{-0.1cm}
{\begin{align}\label{eq:decentralized_problem} 
\begin{split}
\min_{\X \in \bbR^{d\times n}}  &  \frac{1}{n}\sum_{i=1}^n \phi_i(\vx_i), \text{with }\phi_i(\vx_i) \triangleq f_i(\vx_i) + r(\vx_i), \\ % =  \frac{1}{n}\sum_{i=1}^n \left(f_i(\vx_i) + r(\vx_i) \right), \\
 \mbox{s.t.  } \quad & \vx_i=\vx_j, \forall\, j\in \hN_i, \forall\, i = 1,\ldots, n.
\end{split} 
\end{align}}
\vspace{-0.5cm}
%where $\X = [\vx_1,\vx_2,\ldots,\vx_n]\in\bbR^{d\times n}$. In most decentralized computing papers, $r(\vx)=0$ is assumed. We add a nonsmooth regularization here. Therefore, the objective is nonconvex and nonsmooth.

Problems with a \emph{nonsmooth} regularizer, i.e., in the form of \eqref{eq:problem_original}, appear in many applications such as $\ell_1$-regularized signal recovery \cite{eldar2014phase,duchi2019solving}, online nonnegative matrix factorization \cite{guan2012online}, and training sparse neural networks \cite{scardapane2017group, yang2020proxsgd}. When data involved in these applications are distributed onto (or collected by workers on) a decentralized network, it necessitates the design of decentralized algorithms. %for solving equivalent problems in the form of \eqref{eq:decentralized_problem}.

Although decentralized optimization has attracted a lot of research interests in recent years, most existing works focus on strongly convex problems \cite{scaman2017optimal,  koloskova2019decentralized} or convex problems \cite{6426375,taheri2020quantized} or smooth nonconvex problems \cite{bianchi2012convergence, di2016next, wai2017decentralized, lian2017can,zeng2018nonconvex}.
% \YX{A lot of earlier works are missed here.}
Few works have studied \emph{nonsmooth nonconvex} decentralized \emph{stochastic} optimization like \eqref{eq:decentralized_problem} that we consider. \cite{chen2021distributed, xin2021stochastic, mancino2022proximal} are among the exceptions. However, they either require to take many data samples for each update or assume a so-called mean-squared smoothness condition, which is stronger than the smoothness condition in Assumption~\ref{assu:prob}(ii), in order to perform momentum-based variance-reduction step. Though these methods can have convergence (rate) guarantee, they often yield poor generalization performance on training deep neural networks, as demonstrated in  \cite{lecun2012efficient, keskar2016large} for large-batch training methods and in our numerical experiments for momentum variance-reduction methods.
% \PYB{This reads like ours can improve generalization, but I am not sure this is what we want to say. Yes.}

On the other side, many distributed optimization methods \cite{shamir2014distributed,lian2017can,wang2018cooperative} 
% \YX{Give a few references} 
often assume that the data are i.i.d across the workers. %are independent and identically distributed (i.i.d.). But there are cases 
However, this assumption does not hold in many real-world scenarios, for instance, due to data privacy issue that local data has to stay on-premise. %In this case, local data distributions $\{\mathcal{D}_i\}_{i\in[n]}$ are heterogeneous which often gives rise to 
Data heterogeneity can result in significant degradation of the performance by these methods. %in distributed optimization. 
Though some papers do not assume i.i.d. data, they require certain data similarity, such as bounded stochastic gradients \cite{koloskova2019decentralized,koloskova2019decentralized-b, taheri2020quantized} and bounded gradient dissimilarity \cite{ tang2018communication,assran2019stochastic, tang2019deepsqueeze, vogels2020practical}.  
  

To address the critical practical issues mentioned above, we propose a decentralized proximal stochastic gradient tracking method that needs only a single or $O(1)$ data samples (per worker) for each update. With no assumption on data similarity, it can still achieve the optimal convergence rate on solving problems satisfying conditions in Assumption~\ref{assu:prob} and yield good generalization performance. In addition, to reduce communication cost, we give a compressed version of the proposed algorithm, by performing compression on the communicated information. The compressed algorithm can inherit the benefits of its non-compressed counterpart. 

% \JC{Discussions of ``heterogeneous data'' appear to be lacking. What are heterogeneous data? How do they affect analysis and convergence? How do we resolve the challenge? What parts of our bounds are related to heterogeneous data?}

% \JC{It would be good to have some discussions on ``compression.'' How much gain do we get from compression? What compression techniques do we consider? What are the difficulties in applying compression in a stochastic gradient method? How do we resolve these difficulties?}

%When all data are on one machine,  i.e., $n=1$, the problem has been studied in \cite{yang2020proxsgd} and two applications are discussed. One is to train a sparse neural network with $l_1$-regularization, i.e., $\min_{\vx} \bbE_{\xi\sim \mathcal{D}}[F(\vx,\xi)]+\mu\|\vx\|_1$. The other is to train a binary neural network where the model parameters are either $1$ or $-1$ which is achieved by adding a penalty, i.e., $\min_{\vx,\va}  \bbE_{\xi\sim \mathcal{D}}[F(\vx,\xi)]+ \frac{\mu}{4} \sum_{j=1}^d (a_j(x_j+1)^2+(1-a_j)(x_j-1)^2)$ with $\va \in [0,1]^d$, where $\va \in [0,1]^d$ is relaxation of $ a_j = 0  \mbox{ or } 1, j=1,\ldots, d$.  
%These two applications can also been transferred as \eqref{eq:decentralized_problem} and solved by multiple nodes.
  

% Different from widely studied strongly convex \cite{koloskova2019decentralized,liu2020linear,singh2021squarm,song2021optimal} or convex \cite{taheri2020quantized,singh2021squarm,song2022compressed} or smooth \cite{lian2017can,tang2018communication,tang2019deepsqueeze,koloskova2019decentralized-b, taheri2020quantized, singh2021squarm, wang2021error} settings, this paper considers \eqref{eq:decentralized_problem} with smooth but possibily nonconvex $f(\vx)$ and convex but possibily nonsmooth $r(\vx)$. For the possibily nonsmooth term $r(\vx)$, our algorithms include the proximal step \cite{davis2019stochastic,yang2020proxsgd, salzo2021proximal}. The analysis for $r(\vx)=0$ case cannot be directly used to our setting.  \cite{xin2021stochastic} is designed for our setting but need a big batch size which leads to poor generalization \cite{lecun2012efficient, keskar2016large}.
% \cite{mancino2022proximal} is also for our setting and need a small batch size in the iteration except the initial step, but it includes a momentum step which can also leads to poor generalization for large mdoels and large dataset.
% %\red{reference? Currently only find SGD generalizes better than adaptive method \cite{wilson2017marginal, zhou2020towards,xie2021positive}.}
% Our proposed algorithms only need a small batch size without variance reduction and momentum steps.
 

\subsection{Our Contributions}
% \YX{In this section, not only mention what we do, but more importantly, emphasize the advantages of our methods, both in theory and in practice. Also, emphasize the technical challenges.}

Our contributions are three-fold. First, we propose two decentralized algorithms, one without compression (named DProxSGT) and the other with compression (named CDProxSGT), for solving \emph{decentralized nonconvex nonsmooth stochastic} problems. Different from existing methods, e.g., \cite{xin2021stochastic, wang2021distributed, mancino2022proximal}, which need a very large batchsize and/or perform momentum-based variance reduction to handle the challenge from the nonsmooth term, DProxSGT needs only $\mathcal{O}(1)$ data samples for each update, without performing variance reduction. The use of a small batch and a standard proximal gradient update enables our method to achieve significantly better generalization performance over the existing methods, as we demonstrate on training neural networks. To the best of our knowledge, CDProxSGT is the first decentralized algorithm that applies a compression scheme for solving nonconvex nonsmooth stochastic problems, and it inherits the advantages of the non-compressed method DProxSGT. Even applied to the special class of smooth nonconvex problems, CDProxSGT can perform significantly better over state-of-the-art methods, in terms of generalization and handling data heterogeneity.

Second, we establish an optimal sample complexity result of DProxSGT, which matches the lower bound result in \cite{arjevani2022lower} in terms of the dependence on a target tolerance $\epsilon$, to produce an $\epsilon$-stationary solution. Due to the coexistence of nonconvexity, nonsmoothness, big stochasticity variance (due to the small batch and no use of variance reduction for better generalization), and decentralization, the analysis is highly non-trivial. We employ the tool of Moreau envelope and construct a decreasing Lyapunov function by carefully controlling the errors introduced by stochasticity and decentralization. 

Third, we establish the iteration complexity result of the proposed compressed method CDProxSGT, which is in the same order as that for DProxSGT and thus also optimal in terms of the dependence on a target tolerance. The analysis builds on that of DProxSGT but is more challenging due to the additional compression error and the use of gradient tracking. Nevertheless, we obtain our results by making the same (or even weaker) assumptions as those assumed by state-of-the-art methods \cite{koloskova2019decentralized-b, zhao2022beer}. 

% We develop a novel algorithm, DProxSGT, for decentralized nonconvex composite problems.  With the possibly nonsmooth term $r(\vx)$, it is hard to analysis. For the same problem, ProxGT-SA \cite{xin2021stochastic} needs a large batch size of $\frac{1}{\epsilon^2}$ to get an $\epsilon$ stationary point. With variance reduction schemes, ProxGT-SR-O  \cite{xin2021stochastic} and SPPDM \cite{wang2021distributed} still need a batch size of $\frac{1}{\epsilon}$. \cite{mancino2022proximal} reduces the batch size to $\mathcal{O}(1)$, but needs a momentum variance reduction. These methods with large batch size or momentum variance reduction schemes lower down the general accuracy on testing data, which is shown in 
% Section \ref{subsect:RegL1}.
% Our method DProxSGT does not include momentum variance reduction schemes and requires a batch size of only $O(1)$, and it is proved to enjoy the optimal $\mathcal{O}(\frac{1}{\epsilon^4})$ sample complexity and communication complexity which is optimal under Assumption \ref{assu:prob}. The Moreau envelop of $\phi$ is used to analyze the proximal step. Also DProxSGT does not assume the boundedness of the stochastic gradients or the bounded dissimilarity, and can solve decentralized problems with heterogeneous data because of the gradient tracking technique.

% \JC{How does our method differentiate from other methods that solve the same problem (2)?}

% {\color{blue}is there a unique reason to argue for considering the model compression in this case (nonsmooth+compression)? i mean whether the nonsmooth will impose more difficult so we need to address this issue? it is confused  here to motivate this work twice. I suggest to using one example and motivate this work earlier and then discuss the two algorithms.}
 
% To improve the communication efficiency, we propose the compressed version of DProxSGT, CDProxSGT. 
% Current compressed decentralized methods are only for the nonconvex problems with $r\equiv0$, such as \cite{tang2019deepsqueeze, koloskova2019decentralized-b} compress the model parameters, and \cite{zhao2022beer} compresses both the model parameters and tracked gradients. CDProxSGT are designed for \eqref{eq:decentralized_problem} with $r\not\equiv0$. The combination of nonsmooth and compression makes the analysis complex, not only the  Moreau envelop and consensus error, but also compression error need be analyzed. It needs more care to use inequalities and select parameters in the analysis.
% Same as DProxSGT, CDProxSGT enjoys a small batch size and can be used for heterogeneous data without strong assumptions. With compression to save the transmitted amount, CDProxSGT has the same sample complexity and communication complexity as the non-compressed DProxSGT as long as the iteration number is large enough. 

% When $r=0$, CDProxSGT does the similar updates as BEER \cite{zhao2022beer} but BEER \cite{zhao2022beer} needs a larger batchsize and CDProxSGT only needs a batchsize of $\mathcal{O}(1)$ as DProxSGT.  
% In Section \ref{subsect:compress}, the numerical experiments shows that CDProxSGT is comparable with DProxSGT and can obtain higher testing accuracy than BEER.
 


\subsection{Notation}\label{sec:notation}
%\emph{Norms:} %We denote vectors as bold lowercase letters and matrices as bold uppercase letters. 
For any vector $\vx\in\bbR^{d}$, we use $\|\vx\|$ for the $\ell_2$ norm. For any matrix $\A$, $\|\A\|$ denotes the Frobenius norm and $\|\A\|_2$ the spectral norm.
%\emph{Stochastic Gradient}:  
$\X = [\vx_1,\vx_2,\ldots,\vx_n]\in\bbR^{d\times n}$ concatinates all local variables. The superscript $^t$ will be used for iteration or communication.
%We denote 
$\nabla F_i(\vx_i^t,\xi_i^t)$ denotes a local stochastic gradient of $F_i$ at $\vx_i^t$ with a random sample $\xi_i^t$. The column concatenation of $\{\nabla F_i(\vx_i^t,\xi_i^t)\}$ is denoted as 
\vspace{-0.1cm}
\begin{equation*}%\label{eq:gradient_bF} 
\nabla \bF^t = \nabla \bF(\X^t,\Xi^t) = [ \nabla F_1(\vx_1^t,\xi_1^t),\ldots, \nabla F_n(\vx_n^t,\xi_n^t)],\vspace{-0.1cm}
\end{equation*}
where  $\Xi^t = [\xi_1^t,\xi_2^t,\ldots,\xi_n^t]$.
Similarly, we denote %the column concatenation of $\nabla f_i(\vx_i^t)$ as 
\vspace{-0.1cm}
\begin{equation*} 
\nabla \f^t  %= \nabla \f(\X^t) 
= [ \nabla f_1(\vx_1^t ),\ldots, \nabla f_n(\vx_n^t )].\vspace{-0.1cm}
\end{equation*} 
%\emph{Mean}: 
For any $\X \in \bbR^{d\times n}$, %denote its mean along the second dimension, (i.e., the mean among the workers), as 
we define 
\vspace{-0.1cm}
\begin{equation*} \bar{\vx} = \textstyle\frac{1}{n}\X\1, \quad \overline{\X} = \X\J = \bar{\vx}\1^\top,\quad \X_\perp = \X(\I - \J), \vspace{-0.1cm}
\end{equation*} 
where $\1$ is the all-one vector, and $\J = \frac{\1\1^\top}{n}$ is the averaging matrix.
%Also, denote $\J = \frac{\1\1^\top}{n}$, $\overline{\X} = \X\J = \bar{\vx}\1^\top$, and  $\X_\perp = \X(\I - \J)$.
Similarly, we define the mean vectors 
\vspace{-0.1cm}
\begin{equation*} 
\overline{\nabla} \bF^t =  \textstyle\frac{1}{n} \bF^t \1,\ \overline{\nabla} \f^t = \textstyle\frac{1}{n} \f^t \1.\vspace{-0.1cm}
\end{equation*} 
%the mean of  $\nabla \bF^t$ as $\overline{\nabla} \bF^t =  n^{-1}\sum_{i=1}^n \nabla F_i(\vx_i^t,\xi_i^t) $; the mean of  $\nabla \f^t $ as $\overline{\nabla} \f^t =  n^{-1}\sum_{i=1}^n \nabla f_i(\vx_i^t)$.  \\
We will use $\bbE_t$ for the expectation about the random samples $\Xi^t$ at the $t$th iteration and $\bbE$ for the full expectation. $\bbE_Q$ denotes the expectation about a stochastic compressor $Q$.

%\emph{Expectation:} 
%The randomness of Algorithm \ref{alg:DProxSGT} comes from the samples $\{\Xi^t\}_{t\geq 0}$. 
%%\YX{Use $\backslash\mathrm{ldots}$ for $\ldots$ instead of $...$. They look different.}
%The full expectation is denoted as $\bbE$. 
%We assume $\{\xi_i^t\}_{i=1,\ldots,n; t\geq 0}$ are independent to each other. 
%The expectation about the random variables $\Xi^t$ is denoted as $\bbE_t$. %\YX{The notation $\bbE_t$ needs to be defined more clearly.}
%The expectation with respect to the stochastic compressor $Q$ as $\bbE_Q$. 

% Define the proximal mapping as 
% \[
% \prox_{\eta r } (\vx) = \argmin_{y} \{r(\vy)+\frac{1}{2\eta}\|\vy-\vx\|^2\}.
% \]

% \[
% \bar{\nabla} \bF^t, \overline{\nabla} \bF^t, \overline{\nabla \bF}^t, \overline{\nabla \bF^t}
% \]


% \PYB{Make related works a section?}
\section{Related Works}
The literature of decentralized optimization has been growing vastly. To exhaust the literature is impossible. Below we review existing works on decentralized algorithms for solving nonconvex problems, with or without using a compression technique. For ease of understanding the difference of our methods from existing ones, 
we compare to a few relevant methods in Table \ref{tab:method_compare}.

\begin{table*}[t]\label{tab:method_compare}
\caption{Comparison between our methods and some relevant methods: ProxGT-SA and ProxGT-SR-O  in \cite{xin2021stochastic}, DEEPSTORM \cite{mancino2022proximal},  ChocoSGD \cite{koloskova2019decentralized-b}, and  BEER \cite{zhao2022beer}. We %listed the non-compressed methods first then the compressed methods with 
use ``CMP'' to represent whether compression is performed by a method. 
GRADIENTS represents additional assumptions on the stochastic gradients in addition to those made in Assumption \ref{assu:stoc_grad}. 
SMOOTHNESS represents the smoothness condition, where ``mean-squared'' means $\bbE_{\xi_i}[\|\nabla F_i(\vx; \xi_i) - \nabla F_i(\vy; \xi_i)\|^2]\le L^2\|\vx-\vy\|^2$ that is stronger than the $L$-smoothness of $f_i$.
BS is the required batchsize to get an $\epsilon$-stationary solution. VR and MMT represent whether the variance reduction or momentum are used. Large batchsize and/or momentum variance reduction can degrade the generalization performance, as we demonstrate %lower down the model performance on testing data, which will be seen 
in numerical experiments. %ChocoSGD does not need the gradient tracking technique, but it further requires the stochastic gradient be bounded. 
%Our DProxSGT and CDProxSGT do not need means-squared smoothness, and no variance reduction and momentum steps is required under the $\mathcal{O}(1)$ batch size.
% \YX{Add one more column to show if data/gradient similarity or same distribution is assumed.}
}
\label{sample-table}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lccccc}
\toprule
 Methods & CMP & $r\not\equiv 0$  & GRADIENTS  & SMOOTHNESS & (BS, VR, MMT)  \\
\midrule
% \hline
 ProxGT-SA & No& Yes & No & $f_i$ is smooth  &  \big($\mathcal{O}(\frac{1}{\epsilon^2})$, No , No\big) \\[0.1cm]
  ProxGT-SR-O   & No & Yes  & No &  mean-squared &  \big($\mathcal{O}(\frac{1}{\epsilon})$, Yes, No\big)  \\[0.1cm]
  DEEPSTORM  & No & Yes & No &  mean-squared & ($\mathcal{O}(1)$, Yes, Yes)  \\
  \textbf{DProxSGT (this paper)}   & No & Yes & No &  $f_i$ is smooth & ($\mathcal{O}(1)$, No, No)  \\
\midrule
% \hline
   ChocoSGD  & Yes& No & $\bbE_{\xi}[\|\nabla F_i(\vx,\xi_i)\|^2]\leq G^2$   & $f_i$ is smooth & ($\mathcal{O}(1)$, No, No)  \\
   BEER  & Yes & No & No  & $f$ is smooth &  \big($\mathcal{O}(\frac{1}{\epsilon^2})$, No, No\big) \\[0.1cm]
   \textbf{CDProxSGT (this paper)}  & Yes & Yes & No & $f_i$ is smooth & ($\mathcal{O}(1)$, No, No)  \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

% \YX{Let's review the works separately for non-compressed and compressed methods.}
\subsection{Non-compressed Decentralized Methods}
% \YX{Mention works for different settings (only for nonconvex problems): (i) deterministic decentralized methods for regularized problems; (ii) stochastic decentralized methods with/without momentum variance-reduction techniques for smooth problems, i.e., $r=0$; (iii) stochastic decentralized methods with/without momentum variance-reduction techniques for regularized problems. During the review, we can mention gradient tracking that use so that we can handle heterogeneous data, without strong assumptions.}

For nonconvex decentralized problems with a nonsmooth regularizer, a lot of deterministic decentralized methods have been studied, e.g., \cite{di2016next, wai2017decentralized, zeng2018nonconvex, chen2021distributed, scutari2019distributed}.
When only stochastic gradient is available, a majority of existing works focus on smooth cases without a regularizer or a hard constraint, such as \cite{lian2017can, assran2019stochastic, tang2018d}, 
gradient tracking based methods \cite{lu2019gnsd,zhang2019decentralized, koloskova2021improved}, %are for the heterogeneous setting. 
and momentum-based variance reduction methods \cite{xin2021hybrid, zhang2021gt}. %includes some momentum variance reduction schemes. 
% These stochastic methods move model parameters alone the negative of the stochastic gradients or the tracked gradients directly in each iteration, while with the nonsmooth $r(\vx)$, our methods further need a proximal step and we use the Moreau envelop in  analysis.
Several works such as  \cite{bianchi2012convergence, wang2021distributed, xin2021stochastic, mancino2022proximal} have studied stochastic decentralized methods for problems with a nonsmooth term $r$. 
%\YX{What is the difference of these stochastic methods from ours for nonsmooth problems?}
However, they either consider some special $r$ or require a large batch size. \cite{bianchi2012convergence} considers %constrained smooth problems, i.e., 
the case where $r$ is an indicator function of a compact convex set. Also, it %does not include gradient tracking technique and 
requires bounded stochastic gradients. %are bounded in expectation. 
\cite{wang2021distributed} focuses on problems with a polyhedral $r$, and it %when the epigraph of $r$ is a polyhedral set in a special compact form, it is inspired by a proximal augmented Lagrangian method \cite{zhang2020proximal} and 
requires a large batch size of $\mathcal{O}(\frac{1}{\epsilon})$ to produce an (expected) $\epsilon$-stationary point.
\cite{xin2021stochastic, mancino2022proximal} are the most closely related to our methods. To produce an (expected) $\epsilon$-stationary point, the methods in \cite{xin2021stochastic} require a large batch size, either $\mathcal{O}(\frac{1}{\epsilon^2})$ or $\mathcal{O}(\frac{1}{\epsilon})$ if variance reduction is applied. 
The method in \cite{mancino2022proximal} requires only $\mathcal{O}(1)$ samples for each update by taking a momentum-type variance reduction scheme. However, in order to reduce variance, it needs a stronger mean-squared smoothness assumption. In addition, the momentum variance reduction step can often hurt the generalization performance on training complex neural networks, as we will demonstrate in our numerical experiments. %but includes a momentum step when updating the tracked gradients. We can see from our numerical experments that the momentum variacen-reduction techniques can lower down the model performance on testing data when the model is large.

% Our proposed DProxSGT does not need variance reduction schemes or mementum step, and need only $\mathcal{O}(1)$ batchsize. 

   

 % \cite{xin2021stochastic} first provided a unified stochastic proximal gradient tracking framework, ProxGT, where each node first gets a gradient estimation, then does the gradient tracking, proximal update and model average with neighbors in each iteration. When the gradient estimation is based on a batch of samples, it gives ProxGT-SA. When the gradient estimation is based on the variance reduction scheme SARAH \cite{nguyen2017sarah}, it gives ProxGT-SR-O for the case with $f_i(\vx)$ in the expectation form and ProxGT-SR-E  for the case with $f_i(\vx)$ in the finite-sum form. But to get a $\epsilon$ stationary point, a large batch size of $\mathcal{O}(\frac{1}{\epsilon^2})$ is required for ProxGT-SA, and $\mathcal{O}(\frac{1}{\epsilon})$ is required for ProxGT-SR-O, and  $\mathcal{O}(\sqrt{\frac{m}{n}})$ for ProxGT-SR-E with $m$ samples on each node.
 
% \cite{mancino2022proximal} can also solve \eqref{eq:decentralized_problem} with general $r$, and requires only $\mathcal{O}(1)$ batchsize by taking a new variance reduction scheme, and \cite{mancino2022proximal} includes a momentum step when updating the tracked gradients. The momentum step can lower down the model performance on testing data. 
% Our proposed DProxSGT does not need variance reduction schemes or mementum step, and need only $\mathcal{O}(1)$ batchsize. 
 

% Usually, distributed optimization assumes the data on each worker are independent and identically distributed (i.i.d.). But there are cases in real-world scenarios that this assumption does not hold, for instance, due to the data privacy issue that local data has to stay on-premise. In this case, local data distributions $\{\mathcal{D}_i\}_{i\in[n]}$ are heterogeneous which often gives rise to performance degradation in distributed optimization. Some papers do not assume i.i.d. data, but bounded stochastic gradients \cite{koloskova2019decentralized,koloskova2019decentralized-b, taheri2020quantized, singh2021squarm} or bounded gradient dissimilarity \cite{lian2017can, tang2018communication, tang2019deepsqueeze, vogels2020practical, wang2021error}. Our proposed algorithms can be used to heterogeneous data without such assumptions via the gradient tracking steps which have been proved efficient for heterogeneous data \cite{di2016next,nedic2017achieving,lu2019gnsd,pu2020distributed,sun2020improving,xin2021stochastic,song2021optimal,mancino2022proximal,zhao2022beer,DBLP:journals/corr/abs-2202-00255,song2022compressed}.


\subsection{Compressed Distributed Methods}
% \YX{Mention compression technique first, like what it is and why it is important. Then mention works for decentralized methods with compression technique. Also discuss methods separately for different problem classes.}
 

Communication efficiency is a crucial factor when designing a distributed optimization strategy. The current machine learning paradigm oftentimes resorts to models with a large number of parameters, which indicates a high communication cost when the models or gradients are transferred from workers to the parameter server or among workers. This may incur significant latency in training. Hence, communication-efficient algorithms by model or gradient compression have been actively sought.

Two major groups of compression operators are quantization and sparsification. The quantization approaches include 1-bit SGD \cite{seide20141}, SignSGD \cite{bernstein2018signsgd}, QSGD \cite{alistarh2017qsgd}, TernGrad \cite{wen2017terngrad}. The sparsification approaches include Random-$k$ \cite{stich2018sparsified}, Top-$k$ \cite{aji2017sparse}, Threshold-$v$ \cite{dutta2019discrepancy} and ScaleCom \cite{chen2020scalecom}. Direct compression may slow down the convergence especially when compression ratio is high. Error compensation or error-feedback can mitigate the effect by saving the compression error in one communication step and compensating it in the next communication step before another compression \cite{seide20141}. These compression operators are first designed to compress the gradients in the centralized setting \cite{tang2019DoubleSqueeze,karimireddy2019error}.
 
The compression can also be applied to the decentralized setting for smooth problems, i.e., \eqref{eq:decentralized_problem} with $r=0$. \cite{tang2019deepsqueeze} applies the compression with error compensation to the  communication of model parameters in the decentralized seeting.
Choco-Gossip \cite{koloskova2019decentralized} is another communication way to mitigate the slow down effect from compression. It does not compress the model parameters but a residue between  model parameters and its estimation. Choco-SGD uses Choco-Gossip to solve \eqref{eq:decentralized_problem}. BEER \cite{zhao2022beer} includes gradient tracking and compresses both tracked stochastic gradients and model parameters in each iteration by the Choco-Gossip.
BEER needs a large batchsize of $\mathcal{O}(\frac{1}{\epsilon^2})$ in order to produce an $\epsilon$-stationary solution.
DoCoM-SGT\cite{DBLP:journals/corr/abs-2202-00255} does similar updates as BEER but with a momentum term for the update of the tracked gradients, and it only needs an $\mathcal{O}(1)$ batchsize. 

Our proposed CDProxSGT is for solving decentralized problems in the form of \eqref{eq:decentralized_problem} with a nonsmooth $r(\vx)$. To the best of our knowledge, CDProxSGT is the first compressed decentralized method for nonsmooth nonconvex problems without the use of a large batchsize, and it can achieve an optimal sample complexity without the assumption of data similarity or gradient boundedness. 
% \YX{Can we make such a claim?} %with nonzero $r(\vx)$ include both gradient tracking and compression. CDProxSGT does include large batchsize and momentum variance reduction techniques.  

 % {\color{blue}SL you need a table to compare these results more clearly} 

% \PYB{If we separate related works as a new section, move this part to the end of Intro}
